Digital control of negative imaginary systems: a discrete-time hybrid integrator-gain system approach

A hybrid integrator-gain system (HIGS) is a control element that switches between an integrator and a gain, which overcomes some inherent limitations of linear controllers. In this paper, we consider using discrete-time HIGS controllers for the digital control of negative imaginary (NI) systems. We show that the discrete-time HIGS themselves are step-advanced negative imaginary systems. For a minimal linear NI system, there always exists a HIGS controller that can asymptotically stablize it. An illustrative example is provided, where we use the proposed HIGS control method to stabilize a discrete-time mass-spring system.

==> Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
This paper investigates a state feedback stabilization problem using nonlinear NI systems theory for affine nonlinear systems with relative degree less than or equal to two. For such a system that also has a normal form, we provide a state feedback control law that makes it nonlinear NI or OSNI. In this case, if the internal dynamics of the system are ISS, then there exists state feedback control that stabilizes the system. In the case that the system has a nonlinear NI uncertainty, there exists a state feedback control law such that stabilizes the system if a positive definiteness-like assumption is satisfied for the storage function of the closed-loop system. A numerical example is provided to illustrate the process of stabilizing a system with a nonlinear NI uncertainty. Simulation shows that stabilization is achieved, as expected according to the proposed results.

==> Preliminaries.tex <==
\section{PRELIMINARIES}\label{sec:pre}
\begin{lemma}\label{lemma:DT_NI lemma}\cite{ferrante2017discrete}
Let $(A,B,C,D)$ be a minimal state-space realization of a discrete time, symmetric, real, rational, proper transfer function $G(z)$. Suppose $\det (I+A)\neq 0$ and $\det (I-A)\neq 0$. Then, $G(z)$ is NI if and only if there exists a real matrix $X=X^T>0$ such that
\begin{equation}\label{eq:DT_NI lemma}
X-A^TXA\geq 0 \quad \text{and}  \quad C=-B^T(A^T-I)^{-1}X(A+I).	
\end{equation}
\end{lemma}













